Generate What You Prefer: Reshaping Sequential Recommendation via Guided Diffusion

Sequential recommendation aims to recommend the next item that matches a user's interest, based on the sequence of items he/she interacted with before. Scrutinizing previous studies, we can summarize a common learning-to-classify paradigm -- given a positive item, a recommender model performs negative sampling to add negative items and learns to classify whether the user prefers them or not, based on his/her historical interaction sequence. Although effective, we reveal two inherent limitations:(1) it may differ from human behavior in that a user could imagine an oracle item in mind and select potential items matching the oracle; and (2) the classification is limited in the candidate pool with noisy or easy supervision from negative samples, which dilutes the preference signals towards the oracle item. Yet, generating the oracle item from the historical interaction sequence is mostly unexplored. To bridge the gap, we reshape sequential recommendation as a learning-to-generate paradigm, which is achieved via a guided diffusion model, termed DreamRec.Specifically, for a sequence of historical items, it applies a Transformer encoder to create guidance representations. Noising target items explores the underlying distribution of item space; then, with the guidance of historical interactions, the denoising process generates an oracle item to recover the positive item, so as to cast off negative sampling and depict the true preference of the user directly. We evaluate the effectiveness of DreamRec through extensive experiments and comparisons with existing methods. Codes and data are open-sourced at https://github.com/YangZhengyi98/DreamRec.

==> chapters/7_rebuttal.tex <==
\newpage

\begin{table*}[h]
\centering
\caption{ Performance comparison with additional baselines (DiffRec \cite{DiffCF}, DiffuRec \cite{DiffSR_Li}, and CDCR  ec \cite{DiffSR_Yu}). The experiments are conducted 5 times and the average and standard deviation are reported.}
% \vspace{-5px}
\label{tab:exp_main}
\renewcommand\arraystretch{1.2}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccc}
\hline
{\multirow{1}{*}{}}&\multicolumn{2}{c}{YooChoose}&&\multicolumn{2}{c}{KuaiRec}&&\multicolumn{2}{c}{Zhihu} \\  \cline{2-3} \cline{5-6} \cline{8-9}
&HR@20(\%)&NDCG@20(\%)&&HR@20(\%)&NDCG@20(\%)&&HR@20(\%)&NDCG@20(\%) \\\hline
DiffRec&4.33\footnotesize{$\pm$0.02}&1.84\footnotesize{$\pm$0.01}&&3.74\footnotesize{$\pm$0.08}&1.77\footnotesize{$\pm$0.05}&&1.82\footnotesize{$\pm$0.03}&0.65\footnotesize{$\pm$0.09} \\
DiffuRec&3.94\footnotesize{$\pm$0.08}&1.80\footnotesize{$\pm$0.07}&&3.60\footnotesize{$\pm$0.03}&1.37\footnotesize{$\pm$0.07}&&1.59\footnotesize{$\pm$0.04}&0.58\footnotesize{$\pm$0.03} \\
CDCRec&4.28\footnotesize{$\pm$0.03}&1.76\footnotesize{$\pm$0.08}&&4.16\footnotesize{$\pm$0.02}&2.09\footnotesize{$\pm$0.02}&&1.94\footnotesize{$\pm$0.06}&0.69\footnotesize{$\pm$0.04} \\
 \hline
DreamRec&\textbf{4.78}\footnotesize{$\pm$0.06}&\textbf{2.23}\footnotesize{$\pm$0.02}&&\textbf{5.26}\footnotesize{$\pm$0.05}&\textbf{4.11}\footnotesize{$\pm$0.02}&&\textbf{2.26}\footnotesize{$\pm$0.07}&\textbf{0.79}\footnotesize{$\pm$0.01}\\

\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!htbp]
\centering
\caption{Runing time comparison with SASRec. $\text{T}_{\text{training}}$ and $\text{T}_{\text{inference}}$ denote training and inference time per epoch.}
% \vspace{-5px}
\label{tab:exp_main}
\renewcommand\arraystretch{1.2}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccc}
\hline
{\multirow{1}{*}{}}&\multicolumn{2}{c}{YooChoose}&&\multicolumn{2}{c}{KuaiRec}&&\multicolumn{2}{c}{Zhihu} \\  \cline{2-3} \cline{5-6} \cline{8-9}
&$\text{T}_{\text{training}}$&$\text{T}_{\text{inference}}$&&$\text{T}_{\text{training}}$&$\text{T}_{\text{inference}}$&&$\text{T}_{\text{training}}$&$\text{T}_{\text{inference}}$ \\\hline
SASRec&62s&5s&&100s&5s&&8s&1s\\
 \hline
DreamRec&65s&160s&&100s&370s&&8s&5s\\

\hline
\end{tabular}
}
\end{table*}

\vspace{15pt}

\begin{table*}[!htbp]
\centering
\caption{Performance comparison with maximum sequence length as 20.}
% \vspace{-5px}
\label{tab:exp_main}
\renewcommand\arraystretch{1.2}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccc}
\hline
{\multirow{1}{*}{}}&\multicolumn{2}{c}{YooChoose}&&\multicolumn{2}{c}{KuaiRec}&&\multicolumn{2}{c}{Zhihu} \\  \cline{2-3} \cline{5-6} \cline{8-9}
&HR@20(\%)&NDCG(\%)@20&&HR@20(\%)&NDCG@20(\%)&&HR@20(\%)&NDCG@20(\%) \\\hline
SASRec&3.41&1.56&&3.81&1.36&&1.68&0.64 \\
CL4SRec&4.38&1.85&&4.33&1.98&&1.96&0.70 \\
DiffRec&4.29&1.91&&3.66&1.68&&1.87&0.64 \\
 \hline
DreamRec&5.01&2.29&&4.95&4.01&&2.31&0.77\\

\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!htbp]
\centering
\caption{Performance comparison with maximum sequence length as 30.}
% \vspace{-5px}
\label{tab:exp_main}
\renewcommand\arraystretch{1.2}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccc}
\hline
{\multirow{1}{*}{}}&\multicolumn{2}{c}{YooChoose}&&\multicolumn{2}{c}{KuaiRec}&&\multicolumn{2}{c}{Zhihu} \\  \cline{2-3} \cline{5-6} \cline{8-9}
&HR@20(\%)&NDCG@20(\%)&&HR@20(\%)&NDCG@20(\%)&&HR@20(\%)&NDCG@20(\%) \\\hline
SASRec&3.72&1.68&&3.95&1.58&&1.46&0.55 \\
CL4SRec&4.22&1.82&&4.30&1.95&&1.89&0.66 \\
DiffRec&4.17&1.76&&3.72&1.80&&1.74&0.61 \\
 \hline
DreamRec&4.66&1.98&&4.96&4.17&&1.95&0.69\\

\hline
\end{tabular}
}
\end{table*}

\vspace{15pt}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=4.5cm]{fig/tradeoff_yc.pdf}
        % \includegraphics[width=4.5cm]{figure/ks_nominal_sasrec.pdf}
        \caption{YooChoose}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=4.5cm]{fig/tradeoff_ks.pdf}
        \caption{KuaiRec}
    \end{subfigure}        
    \hspace{1mm}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=4.5cm]{fig/tradeoff_zhihu.pdf}
        \caption{Zhihu}
    \end{subfigure}
    \caption{Trade-off between recommendation performance and time cost of inference \wrt total diffusion steps. We can observe that as we increase diffusion steps, the inference time cost increases steadily, while the increasing speed of recommendation performance gets slower. Therefore we should carefully choose the diffusion step in order that the recommendation performance is satisfactory and the time cost of inference is acceptable.}
    \label{fig:exp_visual_ks}
    \vspace{-10pt}
\end{figure}

